Carbon Kagome Nanotubes -- quasi-one-dimensional nanostructures with flat bands

We introduce carbon Kagome nanotubes (CKNTs) -- a new allotrope of carbon formed by rolling up sheets of Kagome graphene, and investigate the properties of this material using first principles calculations. Based on the direction of rolling, we identify two principal varieties of CKNTs -- armchair and zigzag, and find that the bending stiffness associated with rolling Kagome graphene into either type of CKNT is about a third of that associated with rolling conventional graphene into carbon nanotubes (CNTs). Ab initio molecular dynamics simulations indicate that both types of CKNTs are likely to exist as stable structures at room temperature. Each CKNT explored here is metallic and features dispersionless states (i.e., flat bands) throughout its Brillouin zone, along with an associated singular peak in the electronic density of states, close to the Fermi level. We calculate the mechanical and electronic response of CKNTs to torsional and axial strains and compare against conventional CNTs. We show in particular, that upon twisting, degenerate dispersionless electronic states in CKNTs split, Dirac points and partially flat bands emerge from the quadratic band crossing point at the Fermi level, and that these features can be explained using a relatively simple tight-binding model. Overall, CKNTs appear to be unique and striking examples of realistic elemental quasi-one-dimensional (1D) materials that can potentially display fascinating collective material properties arising from the presence of strongly correlated electrons. Additionally, distorted CKNTs may provide an interesting material platform where flat band physics and chirality induced anomalous transport effects may be studied together.

==> Extra.tex <==

In this study, due to the quasi-one-dimensional nature of CKNTs, calculations are carried out using Helical DFT \citep{banerjee2021ab, yu2022density}--- a symmetry-adapted real-space formulation of Kohn-Sham Density Functional Theory. As pointed out in previous works, a key advantage of Helical DFT is the efficient use of representative atoms for any quasi-one-dimensional material with the knowledge of the relevant symmetry group --- usually, just a few are adequate, and the behavior of the system under deformations (small or large) can be obtained by minimizing the system's free energy with respect to the coordinates of the representative atoms.

Nanotubes, in gerneral, are aligned and infinite in extent along \textbf{e\textsubscript{Z}}, which are also of limited extent in the \textbf{e\textsubscript{X}}-\textbf{e\textsubscript{Y}} plane. These geometric constraints suggest that nanotubes can be embedded in an annular cylinder of infinite height and finite radius, referred to as the \textit{global simulation domain}. The structures considered in this work may be undeformed, or more generally, they may include axial deformation (i.e., stretch or compression) along \textbf{e\textsubscript{Z}}, and/or torsional deformation about the same axis. As pointed out in past works, helical and cyclic symmetries can be used to describe such systems conveniently \citep{James_OS, banerjee2021ab, yu2022density, Dumitrica_James_OMD, Pekka_Twisted_GNR, Pekka_CNT_Bending, CNT_Dumitrica} as the orbit of a discrete group of isometries, $\mathcal{G}$ on the set of representative atoms, $\calP$, i.e.,

%Similar to how a single-walled CNT can be rolled from a graphene sheet to a seamless cylinder, \citep{CNT_hamada,CNT_sinnott} CKNTs can be seen as nanotubes formed by rolling a sheet of carbon Kagome graphene. Therefore, the structural optimized carbon Kagome graphene is used for contructing the CKNT from the roll up construction for all CKNT calculatations in this work. CKNTs can be categorized into two principlal varieties depending of the rotational axis of rolling, analogous to CNTs. Figure.\ref{fig:CKNTs} shows the structure of armchair and zigzag CKNTs. One immediate observation that can be made from the figure is the porous size of the walls. By subsituting the hexagonal porous of CNTs with carbon dodegonal structures, the pore diameter had significantly increased. Since porosity fasciliate materials transport through the nanotube sidewalls, such properties could have great impact on material sotrage, electrochemical process and nano-scale filteration design. Benefit from the similarity betweent CNTs and CKNTs, dor the rest of the paper, we will use the chiral indices $(n,m)$ ($n,m \in \Z^{\geq}$ ) to label the type of nanotubes as well as its group order.




Here, the isometry operation (i.e., rigid body motion) consist of the rotation matrix ${\textbf{R}}_{(2\pi m\alpha+n\Theta)}$ with axis \textbf{e\textsubscript{Z}} and translation vector $m\tau \textbf{e\textsubscript{Z}}$. It acts on an arbitrary point $\mathbf{x} \in \mathbb{R}^3$ by rotating it through the angle $2\pi m\alpha+n\Theta$ about the axis of the system, while simultaneously translating it by $m\tau$ about the same axis. The quantity $\mathfrak{N}$ is a natural number that captures any ($\mathfrak{N}$-fold) cyclic symmetries in the nanotube, and the angle $\Theta=2\pi/\mathfrak{N}$. The parameter $\tau$ captures extensions and compressions about the axis, while the scalar $\alpha$ is related to the rate of applied or intrinsic twist in the structure, measured as $\beta = 2\pi\alpha/\tau$. For the CKNTs considered in this work, we have $0\leq\alpha<1$, with $\alpha = 0$ representing untwisted structures. For undeformed armchair and zigzag CKNTs, the value of $\tau$ as suggested by the ``roll-up construction'' \citep{CNT_5, Dumitrica_James_OMD} are $5.137$ Å and $8.897$ Å, respectively (Figure \ref{fig:orth_ckl_rolling}).

which $(\eta,\nu)$ are the symmetry-adapted quantum numbers. $(\eta,\nu)$ are analogous to k points in Cartesian coordinates such that they label the eigenvalues, eigenvectors and the electronic occupations. In the eqation above, $\mathfrak{H}^{\text{KS}}$ denotes the Kohn-Sham operator, $V_{xc}$ denotes the exchange correlation potential, $\Phi$ denotes the net electostatic potential generataed by the electrons and nuclear pseudocharges and $\mathcal{V}_{\text{nl}}$ denotes the non-local psudopotential operator in Kleinman-Bylander form \cite{kleinman1982efficacious}. The governing equations can then be solved using a higher order finite difference scheme with discretization in helical coordiantes \citep{banerjee2021ab, yu2022density}.


using a higher order finite difference scheme formulated using \textit{helical coordinates} \citep{My_PhD_Thesis, banerjee2021ab, yu2022density, ghosh2019symmetry}. 


The aforementioned Helical DFT solves the symmetry adpated Kohn Sham DFT equations within a \textit{fundamental domain} that contains the 12 representative atoms as shown in figure  \ref{fig:orth_ckl_rolling}. Provided that the atoms have radial coordinates within a certain range, the fundamental domain takes the form of a cuboid in helical coordinates. With the geometry of the fundamental domain considered, the symmetry-adapted Kohn-Sham equation can be written as:

\begin{align}
\mathfrak{H}^{\text{KS}}\,\psi_j(\bfx;\eta,\nu) = \lambda_j(\eta,\nu)\,\psi_j(\bfx;\eta,\nu), \;\;
\mathfrak{H}^{\text{KS}} = -\frac{1}{2}\Delta+V_{\text{xc}}+\Phi+\mathcal{V}_{\text{nl}}\,,
\end{align}
which $(\eta,\nu)$ are the symmetry-adapted quantum numbers. $(\eta,\nu)$ are analogous to k points in Cartesian coordinates such that they label the eigenvalues, eigenvectors and the electronic occupations. In the eqation above, $\mathfrak{H}^{\text{KS}}$ denotes the Kohn-Sham operator, $V_{xc}$ denotes the exchange correlation potential, $\Phi$ denotes the net electostatic potential generataed by the electrons and nuclear pseudocharges and $\mathcal{V}_{\text{nl}}$ denotes the non-local psudopotential operator in Kleinman-Bylander form \cite{kleinman1982efficacious}. The governing equations can then be solved using a higher order finite difference scheme with discretization in helical coordiantes \citep{banerjee2021ab, yu2022density}.

The helical DFT calcuations in this work are first carried out by using $h = 0.3$ Bohr, and sampling $15$ k-points in the $\eta$ direction. These discretization choices are sufficient to produce chemically accurate forces and ground state energies for the Troullier-Martins norm conserving pseudopotential \cite{troullier1991efficient} used to model the carbon atoms in this work \citep{yu2022density}. Atomic relaxation is done using the Fast Intertial Relaxation Engine \citep{bitzek2006structural}the relaxation is carried out untill all atomic force components have reached $0.001$ Ha/Bohr or lower. Next, for each relaxed structure, we redo a self-consistent calculation using the finest discretization parameters that within computational resource constraints can be done in a timely manner. This corresponds to a mesh spacing of $h = 0.25$ Bohr and $21$ k-points in the $\eta$-direction.


that in terms of electronic properties, there is no qualitative difference between an LDA versus GGA approach in this work. All reference calculations are done using other standard DFT codes, such as ABINIT and M-SPARC \citep{msparc_xu2020} with same parameters and settings. In addition to the Helical DFT calculations mentioned above, single shot (i.e. without relaxation) calculations with empirical pseudopotential were also done. The emperical pseudopotential calculations are done with the relaxed coordinates obtained from Helical DFT. \textcolor{red}{band structure -- symmetry adapted band diagrams \& DOS calculation}

We calculate the projected Density of States (pDOS) of both the armchair and zigzag CKNTs using Quantum ESPRESSO. The structures and their unit cells were both relaxed using the BFGS algorithm. This resulted is net zero cell stresses and forces of the order of $10^{-5}$ Ha/Bohr per atom. LDA pseudopotentials were used, and Gaussian smearing was applied corresponding to an electronic temperature of $315.77\;K$. The pDOS were calculated in the local atomic XYZ coordinate frame wherein the projections were taken on the atomic oribtals that were rotated to the basis in which the occupation matrix is diagonal.







For all ab initio calculations, we used the Perdew-Wang parametrization \cite{perdew1992accurate} of the Local Density Approximation \citep{KohnSham_DFT}, a $12^{\text{th}}$ order finite difference discretization scheme \citep{chelikowsky1994finite, Chelikowsky_Saad_1,  Chelikowsky_Saad_2, kikuji2005first, ghosh2017sparc_1, ghosh2017sparc_2, ghosh2019symmetry, banerjee2021ab}, vacuum padding of $10$ Bohrs in the radial direction and $1$ milli-Hartree of smearing using the Fermi-Dirac distribution. We observed that in terms of electronic properties, there is no qualitative difference between an LDA versus GGA approach in this work. All reference calculations are done using other standard DFT codes, such as ABINIT and M-SPARC \citep{msparc_xu2020} with same parameters and settings. In addition to the Helical DFT calculations mentioned above, single shot (i.e. without relaxation) calculations with empirical pseudopotential were also done. The emperical pseudopotential calculations are done with the relaxed coordinates obtained from Helical DFT. \textcolor{red}{band structure -- symmetry adapted band diagrams \& DOS calculation}
